Photo-to-Shape Material Transfer for Diverse Structures

We introduce a method for assigning photorealistic relightable materials to 3D shapes in an automatic manner. Our method takes as input a photo exemplar of a real object and a 3D object with segmentation, and uses the exemplar to guide the assignment of materials to the parts of the shape, so that the appearance of the resulting shape is as similar as possible to the exemplar. To accomplish this goal, our method combines an image translation neural network with a material assignment neural network. The image translation network translates the color from the exemplar to a projection of the 3D shape and the part segmentation from the projection to the exemplar. Then, the material prediction network assigns materials from a collection of realistic materials to the projected parts, based on the translated images and perceptual similarity of the materials. One key idea of our method is to use the translation network to establish a correspondence between the exemplar and shape projection, which allows us to transfer materials between objects with diverse structures. Another key idea of our method is to use the two pairs of (color, segmentation) images provided by the image translation to guide the material assignment, which enables us to ensure the consistency in the assignment. We demonstrate that our method allows us to assign materials to shapes so that their appearances better resemble the input exemplars, improving the quality of the results over the state-of-the-art method, and allowing us to automatically create thousands of shapes with high-quality photorealistic materials. Code and data for this paper are available at https://github.com/XiangyuSu611/TMT.

==> figures/gallery.tex <==
\begin{figure}[!t]
	\centering
	\includegraphics[width=\linewidth]{images/gallery2_new.pdf}
	\caption{Gallery of results obtained with our material assignment method. For each example, we show the input exemplar and 3D shape with corresponding semantic projection on columns 1--3, and two views of the material assignment result on columns 4--5. The left half of the figure shows results where the 3D shape and the object in the exemplar are similar to each other, while the right half shows results where the two objects have a larger structural difference. \rh{[update with single column]}}
	\label{fig:gallery}
\end{figure}


==> figures/tab_comp_baseline.tex <==
\begin{table}[!t]%
    \caption{ \rh{Qualitative evaluation of our method comparing to two baselines. [update the evaluation metric with the user study results]}} 
	\label{tab:comp_baseline}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l|l}
				\hline\hline
				\textbf{Methods} &   \textbf{Mat-dis ($\downarrow$)} & \textbf{Mat-acc ($\uparrow$)}&  \textbf{Cat-acc($\uparrow$)} \\ \hline \hline 
				PhotoShape  & 14.03 & 20.09\% &  25.53\%  \\  \hline 
				PhotoShape+ & 15.86 & 14.14\% & 36.20\%  \\  \hline 
				%Baseline 2 & 15.56 & 15.50\% & 37.552\%\\ \hline 
				PhotoShape++ &  \textbf{9.26} & \textbf{28.81\%} & \textbf{48.28\%}  \\ \hline \hline 
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_comp_fine_tune.tex <==
\begin{table}[!t]%
	\caption{Comparison different fine tune strategies. \rh{[This table is currently in low priority. We may run out of time to take all the numbers for this table and need to move it.]}} 
	\label{tab:comp_fine_tune}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{c|c|l|l|l}
				\hline\hline
				\textbf{T-Net} &   \textbf{P-Net} &  \textbf{Mat-dis ($\downarrow$)} & \textbf{Mat-acc ($\uparrow$)}&  \textbf{Sub-acc($\uparrow$)} \\ \hline \hline 
				N & N  & 9.44
 & 28.28\% &  48.04\%  \\  \hline 
				Y & N  & 9.26& 28.81\% & 48.28\%  \\  \hline 
				N & Y & xxx  &  XX\% &   XX\%  \\  \hline 
				Y & Y& \textbf{xxx} & \textbf{XXX\%} & \textbf{XXX\%} \\ \hline \hline 
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_comp_path.tex <==
\begin{table}[!t]%
	\caption{\rh{Comparison of different settings for using the two pairs of images output by the translation network to fine-tune the material predictor. 
                        In our setting, we use two predictors that are first fine-tuned on two types of image pairs separately  and then combine them with the consistency loss to get the best results for ($\hat{O}_t, O_s$) pairs that we use to get the final results, as shown in the last row. \ov{[Should we change to Mat-a, Sub-a, and Mat-d so that it fits in the space?]}}
			%We use Pair 1 + 2 + $L_c$ in our method. %\rh{[Currently, we just succesfully fine-tune the translation network with consistency loss. To be able to fine-tune the prediction network with the consistency loss, we need to make significant change to the code and may run out of time. I will put the number we obtained by only fine-tuning the translation network with consistency loss for now, and the ony problem is that the substance accurarcy is a bit lower than the case without consistency loss.]}
	} 
	\label{tab:comp_path}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l|l|l}
				\hline\hline \textbf{Data} 
		         & \textbf{Predictor} & \textbf{Mat-acc ($\uparrow$)}&  \textbf{Sub-acc($\uparrow$)} &   \textbf{Mat-dis ($\downarrow$)} \\ \hline \hline 
				
				\multirow{2}{*}{\emph{($P_t, \hat{P}_s$)}} 
				 & $\text{Pred}_P$  & 64.87\% &  85.26\%  & 8.31 \\ \cline{2-5} 
				 & $\text{Pred}_P^{*}$  & \textbf{79.17\%} & \textbf{90.41\%} & \textbf{5.24}   \\ \hline \hline
				 
			    
			    \multirow{4}{*}{\emph{($\hat{O}_t, O_s$)}} 
			    & $\text{Pred}_O$  & 10.26\%&  43.83\%  &  16.88 \\ \cline{2-5} 
			    & $\text{Pred}_O^{*}$  & 24.18\%  &  59.71\%  & 12.10  \\\cline{2-5} 
			    & $ L_c (\text{Pred}_P)$  & 26.74\%  &  61.37\%  & 11.67  \\\cline{2-5} 
			    & $  L_c ( \text{Pred}_P^{*})$  & \textbf{26.95\%} & \textbf{62.32\%} & \textbf{11.17}\\ \hline \hline
			
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%





==> figures/tab_comp_path2.tex <==
\begin{table}[!t]%
	\caption{\rh{Comparison of different settings for using the two pairs of images output by the translation network to fine-tune the material predictor. 
			In our setting, we use two predictors that are first fine-tuned on two types of image pairs separately  and then combine them with the consistency loss to get the best results for ($\hat{O}_t, O_s$) pairs that we used to get the final results, as shown in the last row.}
		%We use Pair 1 + 2 + $L_c$ in our method. %\rh{[Currently, we just succesfully fine-tune the translation network with consistency loss. To be able to fine-tune the prediction network with the consistency loss, we need to make significant change to the code and may run out of time. I will put the number we obtained by only fine-tuning the translation network with consistency loss for now, and the ony problem is that the substance accurarcy is a bit lower than the case without consistency loss.]}
	} 
	\label{tab:comp_path}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l|l}
				\hline\hline 
				\textbf{Predictor} & \textbf{Mat-acc ($\uparrow$)}&  \textbf{Sub-acc($\uparrow$)} &   \textbf{Mat-dis ($\downarrow$)} \\ \hline \hline 
				$\text{Pred}_O$  & 10.26\%&  43.83\%  &  16.88 \\  \hline
				$\text{Pred}_O^{*}$  & 24.18\%  &  59.71\%  & 12.10  \\ \hline
				$ L_c (\text{Pred}_O^{*}, \text{Pred}_P)$  & 26.74\%  &  61.37\%  & 11.67  \\ \hline
				$  L_c (\text{Pred}_O^{*},  \text{Pred}_P^{*})$  & \textbf{26.95\%} & \textbf{62.32\%} & \textbf{11.17}\\ \hline \hline
				
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/teaser.tex <==
\begin{teaserfigure}
        \centering
        \caption{Teaser.}
        \label{fig:teaser}
\end{teaserfigure}


==> figures/teaser2.tex <==
\begin{figure*}[!t]
	\centering
	\includegraphics[width=0.99\textwidth]{images/teaser.pdf}
\caption{
     %Results of different shapes given different exemplars. 
        Results of our method PhotoShape++ for transferring materials from exemplars  to 3D shapes.
        We show results generated from different combinations of shapes (given in the left column) and photo exemplars (given in the top row). Note the realism of the assigned materials, the resemblance of the results to the exemplars, and the diversity of structures in the shapes and exemplars. \rh{[need to update with real photo]}
        }
\label{fig:teaser2}
\end{figure*}


==> figures/various_structure.tex <==
\begin{figure}[!t]
	\centering
	\includegraphics[width=\linewidth]{images/various_structure.pdf}
	\caption{
		pairs with large strucural difference.}
	\label{fig:various_structure}
\end{figure}


==> intro_prev.tex <==
\section{Introduction}

% Motivation for the problem
Most applications of computer graphics require 3D shapes with materials, since the geometry of 3D shapes alone does not fully convey the appearance of an object to a human. Shapes with materials are important for rendering realistic 3D scenes, which are relevant in simulations, games, and AR/MR/VR. Materials can include colors and textures, but high-quality realistic materials that can be relit are usually represented as reflectance functions such as BRDFs or SVBRDFs. Moreover, manually assigning realistic materials to 3D meshes can be quite difficult, since the task involves 
%splitting the mesh into patches, possibly parameterizing the patches for 2D texture mapping, and experimentally selecting material parameters for the different patches according to a desired design
experimentally selecting material parameters for patches of a 3D model according to a desired design, possibly also requiring the definition of texture coordinates. Thus, more automated ways of assigning materials to 3D shapes are necessary for mass content creation and customization.

\input{figures/teaser2}

% Alternative approaches other than material assignment
\ov{[If the intro is too long, we cut the first part of this paragraph
and shorten the rest]}
One option to circumvent the problem of material assignment to shapes altogether is the reuse of existing shapes. However, the shapes in many datasets such as ShapeNet and PartNet only contain basic textures but no realistic materials. In addition, shape repositories are not guaranteed to contain the specific shapes that the user requires; the user may need to apply materials to a given 3D model. On the other hand, recently there have been great advances in shape reconstruction with the use of deep learning. Methods have been introduced to reconstruct shapes from different input such as point clouds~\cite{park19,chibane20ndf}, photographs~\cite{ji17surfacenet,han21}, and sketches~\cite{wu17marrnet,delanoy18sketch}.
%with different representations such as volumes~\cite{} and implicit functions~\cite{park19,chen19}. 
Thus, this is a promising direction for the automated creation of shapes. However, in the majority of these methods, materials are not accounted for in the learning and reconstruction, and thus the generated shapes possess only their geometry.

% Introduction to the problem we solve and goals, without too many details on our method yet
In this paper, we introduce a method for automatically assigning realistic materials to 3D shapes to alleviate this gap in the automated creation of 3D shapes. The key idea of our method is to use photos of real objects as exemplars that guide the material assignment (Figure~\ref{fig:teaser}). Similarly to Park \etal~\shortcite{park2018photoshape}, our goal is to automatically produce thousands of \textit{PhotoShapes} (photorealistic relightable 3D shapes) to increase the availability of such models, which are not commonly available. In addition, users can also apply our method to create a PhotoShape from a given 3D shape based on an exemplar photo, where both the shape and exemplar are not part of the datasets that we use for learning. Note that, PhotoShapes, as defined by Park \etal~\shortcite{park2018photoshape}, are not simply textured shapes, but shapes with realistic materials that can be relit, given that they are represented as reflectance functions possibly with additional texture information. As a consequence, the creation of PhotoShapes is also a different problem than simply transferring the texture of a reference photo to a 3D shape~ \cite{wang2016unsupervised,oechsle2019texture}. 

% Challenges of this problem
The creation of PhotoShapes has several challenges of its own. First, in texture transfer, the texture of the input exemplar can be directly transferred to the 3D model after the removal of illumination shading and projection distortions. On the other hand, the assignment of realistic materials requires a mapping from the material in the photograph to a database of reflectance functions, since the photograph itself does not contain such information. The material database needs to be sufficiently diverse. Moreover, the extraction of material information from the exemplar and transfer to the 3D model requires a mapping from the geometry and structure of the object in the 2D exemplar to the geometry and structure of the 3D shape, which is a difficult matching problem.

% Previous work and its limitations
Previous work has studied these problems and introduced methods for shape material assignment and shape reconstruction with materials. As representative examples of previous work, Wang \etal~ \shortcite{wang2016unsupervised} transfer the texture from an exemplar image to a collection of shapes with an alignment method. The notable work of Park \etal~\shortcite{park2018photoshape} uses collections of shapes, materials, and photos to to create thousands of PhotoShapes, where their method uses a CNN to predict material properties for shape segments. Oechsle \etal~\shortcite{oechsle2019texture} learn a spatial function that represents texture information and can be used to assign textures to 3D models, while Hu \etal~\shortcite{hu21pcloud} reconstruct a textured 3D point cloud from a single RGB image. However, most of these methods assume that a good alignment can be obtained between the object in the exemplar and the 3D shape, and thus use local correspondence approaches to compute the part mapping.
Specifically, Park \etal~\shortcite{park2018photoshape} rely heavily on a reliable matching between photos and shapes, which is usually hard to obtain by searching example photos for a given 3D shape. 

% Why our work solves the limitations of previous work and more details
% about our method
In our paper, given a 3D shape with part segmentation and a photo exemplar of a shape from the same object category, we address these limitations so that the shape and object in the photo can have very different geometric structure. We use a state-of-the-art image translation method to establish a mapping between the parts of the two objects, which provides a more robust correspondence between the objects for material transfer. Specifically, the translation method transfers the texture from the exemplar to a projection of the 3D shape, and the part segmentation from the projection to the exemplar (Figure~\ref{fig:overview}). The correspondence can then used to assign materials to the parts of the 3D object, where the materials are similar to those in the parts of the exemplar. In addition, since the translation results in two (texture, segmentation) pairs, we use the two pairs to further ensure the consistency of the material assignment. Finally, we also introduce a more complete material library for mapping from exemplar to reflectance function \ov{[correct?]}\rh{[Their dataset has 453 materials, we have 562, but we deleted some of very similar materials in their dataset and add new ones with more diversity.]}. Given these three improvements, we are able to create thousands of PhotoShapes with materials closer in appearance to the exemplars when compared to the results of previous work. \ov{[Maybe one more sentence about our results or say that the difference is significant]} \rh{[Yes, could also mention the comparisons to other baseline after we complete the result section to be more clear how to describe the improvement. Another improvement is that we consider perceptual similarity between materials during material prediction, and use triplet network to find a better embedded feature space to reflect such similarity thus get more accurate material classification results and smaller perceptual distance than previous method.]}

% Summary of contributions
In summary, our contributions include:
\ov{[Should we add this?]} \rh{[Could add a list to be more clear.]}

